A Hybrid Model-based and Data-driven Approach to Spectrum Sharing in mmWave Cellular Networks

Inter-operator spectrum sharing in millimeter-wave bands has the potential of substantially increasing the spectrum utilization and providing a larger bandwidth to individual user equipment at the expense of increasing inter-operator interference. Unfortunately, traditional model-based spectrum sharing schemes make idealistic assumptions about inter-operator coordination mechanisms in terms of latency and protocol overhead, while being sensitive to missing channel state information. In this paper, we propose hybrid model-based and data-driven multi-operator spectrum sharing mechanisms, which incorporate model-based beamforming and user association complemented by data-driven model refinements. Our solution has the same computational complexity as a model-based approach but has the major advantage of having substantially less signaling overhead. We discuss how limited channel state information and quantized codebook-based beamforming affect the learning and the spectrum sharing performance. We show that the proposed hybrid sharing scheme significantly improves spectrum utilization under realistic assumptions on inter-operator coordination and channel state information acquisition.

==> Ratemflie.tex <==
A = [1	18.6580155915042;
51.049049049049	19.0201220247938;
101.098098098098	18.8640059968701;
151.147147147147	18.9210302887335;
201.196196196196	18.7352436586129;
251.245245245245	18.8291521218106;
301.294294294294	18.873897708586;
351.343343343343	19.0437960298032;
401.392392392392	18.8456120477189;
451.441441441441	19.152958369086;
501.490490490491	18.7287824774204;
551.53953953954	18.9588824876014;
601.588588588589	19.0719665070793;
651.637637637638	18.9025083613543;
701.686686686687	19.2876775761383;
751.735735735736	19.4229798675008;
801.784784784785	19.1353835298042;
851.833833833834	19.4047701692548;
901.882882882883	19.2982289159537;
951.931931931932	19.4390789796852;
1001.98098098098	19.4264531120736;
1052.03003003003	19.2362129377774;
1102.07907907908	19.4399138198705;
1152.12812812813	19.164368672551;
1202.17717717718	19.4546963237979;
1252.22622622623	19.2366867249368;
1302.27527527528	19.4532203639565;
1352.32432432432	19.4286642277032;
1402.37337337337	19.354092223439;
1452.42242242242	19.151918840805;
1502.47147147147	19.1929621469269;
1552.52052052052	19.3045121024456;
1602.56956956957	19.3927455451655;
1652.61861861862	19.2946836602326;
1702.66766766767	20.2874048077583;
1752.71671671672	20.0443800022296;
1802.76576576577	19.9556359716141;
1852.81481481481	19.9853358149058;
1902.86386386386	20.2213603428653;
1952.91291291291	20.0282241236644;
2002.96196196196	20.0337630161358;
2053.01101101101	20.0299122780007;
2103.06006006006	20.0926949078155;
2153.10910910911	20.3340248246133;
2203.15815815816	20.572067818025;
2253.20720720721	20.7245010500323;
2303.25625625626	20.4057994609813;
2353.30530530531	20.7696419529659;
2403.35435435435	20.3732636723977;
2453.4034034034	20.9901184576148;
2503.45245245245	20.6639481004207;
2553.5015015015	20.6889935317724;
2603.55055055055	20.6845939855659;
2653.5995995996	20.7687271693424;
2703.64864864865	20.5755132178792;
2753.6976976977	20.6602445877999;
2803.74674674675	20.571186816598;
2853.7957957958	20.627516000772;
2903.84484484484	20.8858464693845;
2953.89389389389	20.5103786369381;
3003.94294294294	20.7248531190248;
3053.99199199199	20.6457260325326;
3104.04104104104	20.8681836908927;
3154.09009009009	20.5543056467452;
3204.13913913914	20.5895944735955;
3254.18818818819	20.6170296826531;
3304.23723723724	20.6440097544204;
3354.28628628629	20.7453824205221;
3404.33533533534	21.253591295763;
3454.38438438438	21.1872010264364;
3504.43343343343	21.1645039755087;
3554.48248248248	21.5629910850536;
3604.53153153153	21.3916088325208;
3654.58058058058	21.3499988184628;
3704.62962962963	21.4516852928168;
3754.67867867868	21.2808625740913;
3804.72772772773	21.424628292086;
3854.77677677678	21.4753186593441;
3904.82582582583	21.4904788106055;
3954.87487487487	21.3762727211597;
4004.92392392392	21.109955898051;
4054.97297297297	21.2235679856992;
4105.02202202202	21.3188256097485;
4155.07107107107	21.3024705012672;
4205.12012012012	21.4227967921424;
4255.16916916917	21.2875438261098;
4305.21821821822	21.6946611996156;
4355.26726726727	21.7839281749233;
4405.31631631632	21.6254045959132;
4455.36536536537	21.7928785889244;
4505.41441441441	21.6827406642826;
4555.46346346346	21.6959725400921;
4605.51251251251	21.7866661531103;
4655.56156156156	21.9744126657698;
4705.61061061061	21.8543923413184;
4755.65965965966	21.7548132788837;
4805.70870870871	21.8496002278799;
4855.75775775776	21.6549684848703;
4905.80680680681	21.7064963035268;
4955.85585585586	21.7524972434145;
5005.9049049049	21.5779025483059;
5055.95395395395	21.6858649097216;
5106.003003003	21.375937253989;
5156.05205205205	21.7252562610005;
5206.1011011011	21.8157253050653;
5256.15015015015	21.6358083649279;
5306.1991991992	21.8483687429151;
5356.24824824825	21.9407994636474;
5406.2972972973	21.677775271197;
5456.34634634635	21.7211257056764;
5506.3953953954	22.0619052957445;
5556.44444444444	21.7892934822299;
5606.49349349349	21.9623217706914;
5656.54254254254	21.77388743729;
5706.59159159159	21.5847364320772;
5756.64064064064	21.7073960728153;
5806.68968968969	21.5907881299879;
5856.73873873874	21.7838596335992;
5906.78778778779	22.0109498517434;
5956.83683683684	21.6612017569996;
6006.88588588589	21.8062947787467;
6056.93493493493	21.7616327309209;
6106.98398398398	21.9767199519822;
6157.03303303303	21.7765724027024;
6207.08208208208	21.9941962868862;
6257.13113113113	22.2688367874657;
6307.18018018018	22.2440461638299;
6357.22922922923	22.1064454092327;
6407.27827827828	22.0095000684109;
6457.32732732733	22.295107801036;
6507.37637637638	22.23796556195;
6557.42542542543	22.1015827139379;
6607.47447447447	22.1223974898524;
6657.52352352352	22.1425079913968;
6707.57257257257	22.1101572700202;
6757.62162162162	22.1252803530351;
6807.67067067067	22.0729347059992;
6857.71971971972	22.0692828109496;
6907.76876876877	22.161171236007;
6957.81781781782	22.2523526684514;
7007.86686686687	22.0145053502302;
7057.91591591592	22.3681121208894;
7107.96496496496	22.2753622465081;
7158.01401401401	22.3551137413067;
7208.06306306306	22.0551617691387;
7258.11211211211	22.1046991737664;
7308.16116116116	22.1171949478024;
7358.21021021021	22.3803711324497;
7408.25925925926	22.0800874276874;
7458.30830830831	22.1967305290393;
7508.35735735736	22.3089883823338;
7558.40640640641	22.4532712807036;
7608.45545545546	22.0537020605913;
7658.5045045045	22.0994552210339;
7708.55355355355	22.0366087432205;
7758.6026026026	22.2839161753452;
7808.65165165165	22.1057540994637;
7858.7007007007	22.1193078557935;
7908.74974974975	22.1452446591938;
7958.7987987988	22.1170411471093;
8008.84784784785	22.0747636571614;
8058.8968968969	22.1456244951095;
8108.94594594595	22.1604123011462;
8158.994994995	22.0205204110232;
8209.04404404404	22.1712510397739;
8259.09309309309	22.135343751013;
8309.14214214214	22.1388215646448;
8359.19119119119	22.0688650228819;
8409.24024024024	22.2946306911091;
8459.28928928929	22.2280099724197;
8509.33833833834	22.9786912388989;
8559.38738738739	23.0539995642327;
8609.43643643644	22.8595875173634;
8659.48548548549	22.7800980967944;
8709.53453453453	22.9994627035975;
8759.58358358358	22.8821964254157;
8809.63263263263	22.9018961649636;
8859.68168168168	23.2301449569944;
8909.73073073073	22.645440576036;
8959.77977977978	23.0352900506378;
9009.82882882883	23.0891453476253;
9059.87787787788	22.8598996181321;
9109.92692692693	22.8258363960328;
9159.97597597598	23.0234660498119;
9210.02502502502	22.8528008143782;
9260.07407407407	22.8462125179299;
9310.12312312312	22.9424338280001;
9360.17217217217	22.9531587896546;
9410.22122122122	23.1377526528261;
9460.27027027027	22.8857171556299;
9510.31931931932	23.1421813534048;
9560.36836836837	22.7558588719411;
9610.41741741742	22.7938621047465;
9660.46646646647	22.8472540751969;
9710.51551551552	22.9731725125913;
9760.56456456457	22.9062185261275;
9810.61361361361	22.9193992516862;
9860.66266266266	22.7833059790065;
9910.71171171171	22.7073316310506;
9960.76076076076	23.1474412273621;
10010.8098098098	22.8621889001808;
10060.8588588589	22.8483932084514;
10110.9079079079	22.9461159755793;
10160.956956957	22.7871254780559;
10211.006006006	22.7460117897024;
10261.0550550551	23.2370922757198;
10311.1041041041	23.0698955786543;
10361.1531531532	22.8189135455513;
10411.2022022022	22.9752542624624;
10461.2512512513	23.4258197773023;
10511.3003003003	23.1232492972272;
10561.3493493493	23.126014116417;
10611.3983983984	22.9977733501185;
10661.4474474474	23.1782572626292;
10711.4964964965	23.1311112729361;
10761.5455455455	22.9655291332619;
10811.5945945946	23.079651059349;
10861.6436436436	23.2014841133547;
10911.6926926927	23.204744080454;
10961.7417417417	22.9903374865077;
11011.7907907908	23.240504017003;
11061.8398398398	23.4247625122733;
11111.8888888889	23.044541399156;
11161.9379379379	23.0344920935956;
11211.986986987	23.1615037303103;
11262.036036036	23.2490997367565;
11312.0850850851	23.1920397464079;
11362.1341341341	23.612091276336;
11412.1831831832	23.1039316859866;
11462.2322322322	23.3375052271291;
11512.2812812813	23.3202743439052;
11562.3303303303	23.2404210589652;
11612.3793793794	23.1789943584414;
11662.4284284284	23.2648670534927;
11712.4774774775	23.0909067448293;
11762.5265265265	23.3656749680669;
11812.5755755756	23.3632695515887;
11862.6246246246	22.876652194779;
11912.6736736737	23.3126550322249;
11962.7227227227	23.4067480755923;
12012.7717717718	23.3001611994268;
12062.8208208208	23.5124475305629;
12112.8698698699	23.4245927957507;
12162.9189189189	23.3256031915751;
12212.967967968	23.2726298225927;
12263.017017017	23.4482851912568;
12313.0660660661	23.3080455404542;
12363.1151151151	23.3373209152104;
12413.1641641642	22.918921152903;
12463.2132132132	23.386520169984;
12513.2622622623	23.4726009859627;
12563.3113113113	23.3815266522939;
12613.3603603604	23.4198193593873;
12663.4094094094	23.5573418155794;
12713.4584584585	23.3363930498233;
12763.5075075075	23.428118465202;
12813.5565565566	23.3155760036279;
12863.6056056056	23.3373711571765;
12913.6546546547	23.5134769974466;
12963.7037037037	23.3973287896854;
13013.7527527528	23.5254761047142;
13063.8018018018	23.4982604552511;
13113.8508508509	23.4808082130736;
13163.8998998999	23.2501515321994;
13213.9489489489	23.5558198003501;
13263.997997998	23.5463834825002;
13314.047047047	23.2927005399956;
13364.0960960961	23.3719304147519;
13414.1451451451	23.2798359027036;
13464.1941941942	23.4166141569362;
13514.2432432432	23.3342983521559;
13564.2922922923	23.2634627500541;
13614.3413413413	23.2499064912325;
13664.3903903904	23.2648114797044;
13714.4394394394	23.2402964612387;
13764.4884884885	23.5835217399512;
13814.5375375375	23.2625937642937;
13864.5865865866	23.2672666676854;
13914.6356356356	23.2758786873315;
13964.6846846847	23.3938681235093;
14014.7337337337	23.3138933107051;
14064.7827827828	23.3332204334906;
14114.8318318318	23.7624278212053;
14164.8808808809	23.466612277431;
14214.9299299299	23.1094461080648;
14264.978978979	23.3236131642273;
14315.028028028	23.2905548960955;
14365.0770770771	23.2330571044866;
14415.1261261261	23.5348768316692;
14465.1751751752	23.5059754482922;
14515.2242242242	23.4368405850076;
14565.2732732733	23.4689011701947;
14615.3223223223	23.6024947307473;
14665.3713713714	23.5801026316744;
14715.4204204204	23.1694164998747;
14765.4694694695	23.5675620952642;
14815.5185185185	23.5162086440631;
14865.5675675676	23.324279915723;
14915.6166166166	23.2982906931143;
14965.6656656657	23.5552870666882;
15015.7147147147	23.4589422088775;
15065.7637637638	23.4063351644079;
15115.8128128128	23.4450228316274;
15165.8618618619	23.3726372194387;
15215.9109109109	23.2191855281393;
15265.95995996	23.2760611415888;
15316.009009009	23.3183950000045;
15366.0580580581	23.3365621291179;
15416.1071071071	23.2827819358622;
15466.1561561562	23.278891833708;
15516.2052052052	23.5104460792655;
15566.2542542543	23.4585223913963;
15616.3033033033	23.3978374641013;
15666.3523523524	23.4464571059568;
15716.4014014014	23.5543339458203;
15766.4504504505	23.4212880907303;
15816.4994994995	23.3022206122361;
15866.5485485485	23.3408116569486;
15916.5975975976	23.3236587248065;
15966.6466466466	23.4963740316119;
16016.6956956957	23.4298293449413;
16066.7447447447	23.3389273510828;
16116.7937937938	23.2433433629852;
16166.8428428428	23.5486512503896;
16216.8918918919	23.4283207921089;
16266.9409409409	23.3412793891087;
16316.98998999	23.640470745988;
16367.039039039	23.602951042045;
16417.0880880881	23.2433117079619;
16467.1371371371	23.2158396071497;
16517.1861861862	23.5703676573678;
16567.2352352352	23.5780680283525;
16617.2842842843	23.2621574099424;
16667.3333333333	23.4423570570054;
16717.3823823824	23.515910613915;
16767.4314314314	23.3418968482359;
16817.4804804805	23.332212246344;
16867.5295295295	23.3070036188707;
16917.5785785786	23.429136544498;
16967.6276276276	23.3520241550376;
17017.6766766767	23.3990542770873;
17067.7257257257	23.6094382848799;
17117.7747747748	23.4413473192021;
17167.8238238238	23.2539248940441;
17217.8728728729	23.1098055137756;
17267.9219219219	23.45283323055;
17317.970970971	23.2289882913548;
17368.02002002	23.3070973716514;
17418.0690690691	23.268789927841;
17468.1181181181	23.6776350532998;
17518.1671671672	23.6274879730498;
17568.2162162162	23.4668504362251;
17618.2652652653	23.8766929137906;
17668.3143143143	23.8058935058642;
17718.3633633634	23.3267772495294;
17768.4124124124	23.8037924670323;
17818.4614614615	23.7454241940559;
17868.5105105105	23.6103525003705;
17918.5595595596	23.6894303472313;
17968.6086086086	23.5467006284775;
18018.6576576577	23.6686537820879;
18068.7067067067	23.8737826652688;
18118.7557557558	23.7126710671095;
18168.8048048048	23.627529333281;
18218.8538538539	23.6194562517669;
18268.9029029029	23.8160033679528;
18318.951951952	23.912558361951;
18369.001001001	23.6466698999289;
18419.05005005	23.532539879176;
18469.0990990991	23.5865865021638;
18519.1481481481	23.6173652095332;
18569.1971971972	23.7537650287571;
18619.2462462462	23.3716909414191;
18669.2952952953	23.7083687904509;
18719.3443443443	23.6662154765162;
18769.3933933934	23.5739900337832;
18819.4424424424	23.8593377120866;
18869.4914914915	23.4919822568547;
18919.5405405405	23.6761769950033;
18969.5895895896	23.7478224191154;
19019.6386386386	23.6808263720482;
19069.6876876877	23.7394687865404;
19119.7367367367	23.6724909041236;
19169.7857857858	23.5844865564263;
19219.8348348348	23.793098486407;
19269.8838838839	23.8468185453385;
19319.9329329329	23.8370028761555;
19369.981981982	23.6839112507161;
19420.031031031	23.6717045132973;
19470.0800800801	24.0057632019316;
19520.1291291291	23.5997749056875;
19570.1781781782	23.5524080287193;
19620.2272272272	23.4725881798195;
19670.2762762763	23.6529419528141;
19720.3253253253	23.5977253611596;
19770.3743743744	23.8738724812153;
19820.4234234234	23.6572645307976;
19870.4724724725	23.803283843377;
19920.5215215215	23.787602209363;
19970.5705705706	23.5324489334132;
20020.6196196196	23.8914011642928;
20070.6686686687	23.7266477984239;
20120.7177177177	23.7819280745783;
20170.7667667668	23.7419118129948;
20220.8158158158	23.8064198109397;
20270.8648648649	23.5078536648396;
20320.9139139139	23.5786565652402;
20370.962962963	23.9050979774735;
20421.012012012	23.7265949535303;
20471.0610610611	23.7395815041491;
20521.1101101101	23.8433632662984;
20571.1591591592	23.7085835164683;
20621.2082082082	23.8277208246194;
20671.2572572573	23.9707717386422;
20721.3063063063	23.5233932346263;
20771.3553553554	23.8032184185251;
20821.4044044044	23.7594699557893;
20871.4534534535	23.8451786779341;
20921.5025025025	23.7005220953647;
20971.5515515516	23.5234622982418;
21021.6006006006	23.7682629271616;
21071.6496496497	23.7361832067185;
21121.6986986987	23.5551777264458;
21171.7477477477	23.9055322674884;
21221.7967967968	23.6072167984383;
21271.8458458458	23.6048387217786;
21321.8948948949	23.5549216954869;
21371.9439439439	23.6628375464132;
21421.992992993	23.6548319487021;
21472.042042042	23.736548508219;
21522.0910910911	23.6301470459195;
21572.1401401401	23.827828161072;
21622.1891891892	23.5719010881324;
21672.2382382382	23.7522514116004;
21722.2872872873	23.5991151084801;
21772.3363363363	23.9775382570669;
21822.3853853854	23.6930671945423;
21872.4344344344	24.1473220516894;
21922.4834834835	23.6662824119777;
21972.5325325325	23.6583931189068;
22022.5815815816	23.8513578815232;
22072.6306306306	23.7939659915515;
22122.6796796797	23.5002731830538;
22172.7287287287	23.8389526223695;
22222.7777777778	23.9886646894774;
22272.8268268268	23.7290044525856;
22322.8758758759	23.9167955648771;
22372.9249249249	23.8220318839436;
22422.973973974	23.7579941322074;
22473.023023023	23.629148521092;
22523.0720720721	23.6233190720515;
22573.1211211211	23.8338183708022;
22623.1701701702	23.629947010101;
22673.2192192192	23.519414771148;
22723.2682682683	23.9576728753476;
22773.3173173173	23.8032099653378;
22823.3663663664	23.8831474499087;
22873.4154154154	24.1093988375979;
22923.4644644645	23.8356360317373;
22973.5135135135	23.9837527347958;
23023.5625625626	23.8700025128745;
23073.6116116116	23.6135425068812;
23123.6606606607	23.9060010642672;
23173.7097097097	23.3876313386729;
23223.7587587588	23.9433367506909;
23273.8078078078	23.7420711201241;
23323.8568568569	23.7371049935923;
23373.9059059059	23.6920999072654;
23423.954954955	23.7115753955594;
23474.004004004	23.7478397620929;
23524.0530530531	23.7821129162596;
23574.1021021021	23.5822029307738;
23624.1511511512	23.9155600982412;
23674.2002002002	23.6483675638616;
23724.2492492492	23.8199904742194;
23774.2982982983	23.7225890712322;
23824.3473473473	23.5774908250849;
23874.3963963964	23.8020846072372;
23924.4454454454	23.5899581747408;
23974.4944944945	23.7654407029896;
24024.5435435435	23.8913041423155;
24074.5925925926	23.5722163809294;
24124.6416416416	23.6618774847465;
24174.6906906907	23.8772257290638;
24224.7397397397	23.8571871537235;
24274.7887887888	23.6726374077024;
24324.8378378378	23.7552072527323;
24374.8868868869	23.7151294556844;
24424.9359359359	23.7419952607276;
24474.984984985	24.014074776384;
24525.034034034	23.636149815304;
24575.0830830831	23.5676887376445;
24625.1321321321	23.5996226508417;
24675.1811811812	23.8546100919483;
24725.2302302302	23.7963539549331;
24775.2792792793	23.8147342198031;
24825.3283283283	23.6300166227324;
24875.3773773774	24.0361610761951;
24925.4264264264	23.8703075898384;
24975.4754754755	24.0016589566928;
25025.5245245245	23.8903881637262;
25075.5735735736	23.8010097862774;
25125.6226226226	23.8444106483827;
25175.6716716717	23.9799658366615;
25225.7207207207	23.7889545784585;
25275.7697697698	23.8104510681021;
25325.8188188188	23.6840713699742;
25375.8678678679	23.71341081984;
25425.9169169169	23.9763612844895;
25475.965965966	23.6281233627924;
25526.015015015	23.9439438699788;
25576.0640640641	23.7866730109145;
25626.1131131131	23.5333723640757;
25676.1621621622	23.5894380803188;
25726.2112112112	23.7823183563009;
25776.2602602603	23.8315691700801;
25826.3093093093	23.7325116331901;
25876.3583583584	23.7194084612787;
25926.4074074074	23.7439650464372;
25976.4564564565	23.4606662045025;
26026.5055055055	23.5272602410327;
26076.5545545546	23.8026712166982;
26126.6036036036	23.7742122458626;
26176.6526526527	23.8683802573461;
26226.7017017017	23.7468324147978;
26276.7507507508	23.9620796715739;
26326.7997997998	23.6185477962028;
26376.8488488488	23.6142556442332;
26426.8978978979	23.695109499285;
26476.9469469469	24.030406089801;
26526.995995996	23.7809926060138;
26577.045045045	23.7760285038727;
26627.0940940941	23.599455218565;
26677.1431431431	23.8386869183421;
26727.1921921922	23.8731188157852;
26777.2412412412	23.9737074192995;
26827.2902902903	23.7573199941616;
26877.3393393393	23.8862463979091;
26927.3883883884	23.8662813172712;
26977.4374374374	23.4919531232231;
27027.4864864865	23.785971265088;
27077.5355355355	23.6470201330142;
27127.5845845846	23.8298024862157;
27177.6336336336	23.9841589390924;
27227.6826826827	23.578451849613;
27277.7317317317	23.7923549103846;
27327.7807807808	23.643872821295;
27377.8298298298	23.5776662973259;
27427.8788788789	23.6339781093595;
27477.9279279279	23.6758119881051;
27527.976976977	23.9585216429809;
27578.026026026	23.8222541805652;
27628.0750750751	23.937330778475;
27678.1241241241	23.614459831992;
27728.1731731732	23.7254029773994;
27778.2222222222	23.7871533345859;
27828.2712712713	23.8220051651189;
27878.3203203203	24.0224694401874;
27928.3693693694	23.8296297941391;
27978.4184184184	23.8661082087431;
28028.4674674675	23.8416826933738;
28078.5165165165	24.0450038570547;
28128.5655655656	23.8719601215964;
28178.6146146146	23.9763388517647;
28228.6636636637	23.6400294493546;
28278.7127127127	23.7405724797555;
28328.7617617618	23.6134482469331;
28378.8108108108	23.7764166771547;
28428.8598598599	23.5337408946534;
28478.9089089089	23.4679786579539;
28528.957957958	23.6976903770507;
28579.007007007	23.6906615023446;
28629.0560560561	23.83420611242;
28679.1051051051	23.6841293632804;
28729.1541541542	23.6902038942536;
28779.2032032032	23.7432035745318;
28829.2522522523	23.7892244099492;
28879.3013013013	23.6677705198268;
28929.3503503503	23.6816344787687;
28979.3993993994	23.7906271691448;
29029.4484484484	23.6537056856001;
29079.4974974975	23.5362402987183;
29129.5465465465	23.8985260571332;
29179.5955955956	23.7296852669022;
29229.6446446446	23.7895435676635;
29279.6936936937	23.7387563042532;
29329.7427427427	23.6235229196876;
29379.7917917918	23.7380071961524;
29429.8408408408	23.9870745053842;
29479.8898898899	23.5069634802723;
29529.9389389389	23.7066186422381;
29579.987987988	23.8547584827535;
29630.037037037	23.7768013841842;
29680.0860860861	23.6323432294142;
29730.1351351351	23.7983657247993;
29780.1841841842	23.8507487885547;
29830.2332332332	23.7187718182585;
29880.2822822823	23.7188957858875;
29930.3313313313	23.8919840629903;
29980.3803803804	23.9398982672004;
30030.4294294294	23.9140414247496;
30080.4784784785	23.6855714247692;
30130.5275275275	24.0391349333403;
30180.5765765766	23.7980342152692;
30230.6256256256	23.6734228847345;
30280.6746746747	23.5754465921602;
30330.7237237237	24.0697051955718;
30380.7727727728	23.6278789403037;
30430.8218218218	23.6701608776849;
30480.8708708709	23.9073615770944;
30530.9199199199	23.705462305767;
30580.968968969	23.5960360727381;
30631.018018018	23.7571114468129;
30681.0670670671	23.7189524093071;
30731.1161161161	23.7388903939074;
30781.1651651652	23.8609200728998;
30831.2142142142	23.8458190564746;
30881.2632632633	23.6187674639463;
30931.3123123123	23.7199999924082;
30981.3613613614	23.7780951660329;
31031.4104104104	23.96682642431;
31081.4594594595	23.7528854453366;
31131.5085085085	23.7231061934893;
31181.5575575576	24.1033388237122;
31231.6066066066	23.7199512013756;
31281.6556556557	23.9901367070745;
31331.7047047047	23.9322857327043;
31381.7537537538	23.7336243972799;
31431.8028028028	23.7549823305669;
31481.8518518519	23.8460753157159;
31531.9009009009	23.7575998011669;
31581.94994995	23.9627995749573;
31631.998998999	23.9543112210713;
31682.048048048	23.9077663411839;
31732.0970970971	23.9534889596194;
31782.1461461461	23.708603961449;
31832.1951951952	23.8405532500895;
31882.2442442442	23.778918837;
31932.2932932933	23.5996440602837;
31982.3423423423	23.8605349213477;
32032.3913913914	23.7958987959307;
32082.4404404404	23.8588503651802;
32132.4894894895	23.8002916962227;
32182.5385385385	23.8984258072054;
32232.5875875876	23.8752232538392;
32282.6366366366	23.8078772272495;
32332.6856856857	23.4691307481338;
32382.7347347347	23.866666025888;
32432.7837837838	23.7381969765089;
32482.8328328328	23.664589131299;
32532.8818818819	23.8471774752183;
32582.9309309309	23.8343999071804;
32632.97997998	23.8044216984405;
32683.029029029	23.4740080394917;
32733.0780780781	24.1822885031168;
32783.1271271271	23.9877824195807;
32833.1761761762	23.8599891794942;
32883.2252252252	23.8069181797383;
32933.2742742743	23.9381101660531;
32983.3233233233	23.6792845041298;
33033.3723723724	23.9262278142457;
33083.4214214214	23.8110580940988;
33133.4704704705	23.8007238085251;
33183.5195195195	24.0649795377787;
33233.5685685686	23.9409400018985;
33283.6176176176	23.9856948128715;
33333.6666666667	23.6695580756865;
33383.7157157157	23.7899453070209;
33433.7647647648	23.9369113260257;
33483.8138138138	23.827092062512;
33533.8628628629	23.9479176350583;
33583.9119119119	23.6353459103418;
33633.960960961	23.7130589971083;
33684.01001001	23.7986338353067;
33734.0590590591	23.7408265158838;
33784.1081081081	23.7361538594625;
33834.1571571572	24.0369295687033;
33884.2062062062	23.5987600776503;
33934.2552552553	23.5681911408435;
33984.3043043043	23.8931207624524;
34034.3533533534	23.6102709847063;
34084.4024024024	23.9584770157639;
34134.4514514515	23.9062805218602;
34184.5005005005	23.8515540162335;
34234.5495495495	23.8489649583407;
34284.5985985986	23.7307356273115;
34334.6476476476	23.7950028153762;
34384.6966966967	23.6261830573077;
34434.7457457457	23.8828036671935;
34484.7947947948	23.8457279839821;
34534.8438438438	23.7700631264603;
34584.8928928929	23.9539723982503;
34634.9419419419	23.924170774664;
34684.990990991	24.0389807736256;
34735.04004004	23.8024863290426;
34785.0890890891	23.860480443346;
34835.1381381381	23.7661586760646;
34885.1871871872	23.763562412276;
34935.2362362362	24.1017216331697;
34985.2852852853	23.8530107819841;
35035.3343343343	23.8463399785239;
35085.3833833834	23.7880706483803;
35135.4324324324	23.4891255711975;
35185.4814814815	24.09846968216;
35235.5305305305	23.7803510637349;
35285.5795795796	23.8905613784098;
35335.6286286286	23.8018212121488;
35385.6776776777	23.8489598531912;
35435.7267267267	23.6856540297491;
35485.7757757758	23.7172123912927;
35535.8248248248	23.4848078119884;
35585.8738738739	23.9020567650468;
35635.9229229229	23.8960201709461;
35685.971971972	23.8088637975812;
35736.021021021	23.6536877932583;
35786.0700700701	23.6707581836077;
35836.1191191191	23.888590642741;
35886.1681681682	23.6876394977165;
35936.2172172172	24.0022496132817;
35986.2662662663	23.714501019734;
36036.3153153153	23.8648581524177;
36086.3643643644	23.7181633979855;
36136.4134134134	23.9214805181322;
36186.4624624625	23.744822573686;
36236.5115115115	23.7634501176607;
36286.5605605606	23.7511970235228;
36336.6096096096	23.7286180458127;
36386.6586586587	23.788237266148;
36436.7077077077	23.6831020011865;
36486.7567567568	23.783259745973;
36536.8058058058	23.4663746859325;
36586.8548548549	23.565150851306;
36636.9039039039	23.7674222062414;
36686.952952953	23.7973777883576;
36737.002002002	23.6123754978873;
36787.0510510511	23.7573634805289;
36837.1001001001	23.9385266225795;
36887.1491491491	23.937171635157;
36937.1981981982	23.7293795650545;
36987.2472472472	23.6463669172106;
37037.2962962963	23.6366386497691;
37087.3453453453	23.9080386647062;
37137.3943943944	23.8640444461086;
37187.4434434434	23.6459466347481;
37237.4924924925	23.8292574462988;
37287.5415415415	23.7962876978945;
37337.5905905906	23.9648112435545;
37387.6396396396	23.5797969026895;
37437.6886886887	23.8112759689786;
37487.7377377377	23.6816751361895;
37537.7867867868	23.7550548488718;
37587.8358358358	23.8565042254741;
37637.8848848849	23.9089413876829;
37687.9339339339	23.5771402902653;
37737.982982983	23.6971392962183;
37788.032032032	23.3952237765282;
37838.0810810811	23.7355504860272;
37888.1301301301	23.8992776420476;
37938.1791791792	23.739590245718;
37988.2282282282	23.8972377376;
38038.2772772773	23.9409608721507;
38088.3263263263	24.2888704836335;
38138.3753753754	24.0033797022417;
38188.4244244244	23.7809623443435;
38238.4734734735	23.7101873919538;
38288.5225225225	23.8260817660803;
38338.5715715716	23.6773294823068;
38388.6206206206	23.8587546351203;
38438.6696696697	23.7295320330402;
38488.7187187187	23.8441222156869;
38538.7677677678	23.777307309629;
38588.8168168168	23.6796747741911;
38638.8658658659	23.7873204073916;
38688.9149149149	23.8658109924332;
38738.963963964	23.6205329219648;
38789.013013013	23.6900305580172;
38839.0620620621	23.8446080605731;
38889.1111111111	23.8968651446792;
38939.1601601602	23.8943060917923;
38989.2092092092	23.7274739830965;
39039.2582582583	24.0054591174241;
39089.3073073073	23.675906900229;
39139.3563563564	23.9132127070907;
39189.4054054054	23.9837521782842;
39239.4544544545	23.6516922401118;
39289.5035035035	23.7655551798355;
39339.5525525526	23.8415998846049;
39389.6016016016	23.8034323780222;
39439.6506506506	23.8242864591986;
39489.6996996997	23.7022777752834;
39539.7487487487	23.9732796883199;
39589.7977977978	23.8374181647209;
39639.8468468468	23.7547662774781;
39689.8958958959	23.756456679407;
39739.9449449449	23.6410452849683;
39789.993993994	23.686403770038;
39840.043043043	23.9035949864521;
39890.0920920921	23.712115548659;
39940.1411411411	23.9242401985857;
39990.1901901902	24.0570951951957;
40040.2392392392	23.943145181376;
40090.2882882883	23.8443413991831;
40140.3373373373	23.8921413650861;
40190.3863863864	24.0007452731225;
40240.4354354354	23.5857260754736;
40290.4844844845	23.8724592965139;
40340.5335335335	23.8464736367799;
40390.5825825826	23.7522573249497;
40440.6316316316	23.8314414076845;
40490.6806806807	23.755005488631;
40540.7297297297	23.8285228009991;
40590.7787787788	23.6292482852691;
40640.8278278278	23.6138366042792;
40690.8768768769	23.7202712825188;
40740.9259259259	23.8053419804311;
40790.974974975	24.0045023927217;
40841.024024024	23.8713279193349;
40891.0730730731	23.9378900749893;
40941.1221221221	23.5494901640532;
40991.1711711712	23.8741801841249;
41041.2202202202	23.9797725958752;
41091.2692692693	23.6110041163632;
41141.3183183183	23.852901083609;
41191.3673673674	24.0547279108345;
41241.4164164164	23.9626463037319;
41291.4654654655	23.9689126036566;
41341.5145145145	23.8817833170843;
41391.5635635636	23.6849069443659;
41441.6126126126	23.6551967638953;
41491.6616616617	23.7587898338372;
41541.7107107107	23.6404847809396;
41591.7597597598	24.0783601799527;
41641.8088088088	23.8449176530177;
41691.8578578579	23.8192399402083;
41741.9069069069	23.9761599455332;
41791.955955956	23.8785682522237;
41842.005005005	23.7474088666534;
41892.0540540541	23.6854449921024;
41942.1031031031	23.9276838817901;
41992.1521521521	23.8313753816212;
42042.2012012012	23.7833613328712;
42092.2502502503	23.6450055429939;
42142.2992992993	23.7419828839101;
42192.3483483484	23.7221152538574;
42242.3973973974	23.7329418819337;
42292.4464464464	23.8976976161081;
42342.4954954955	23.9030492434804;
42392.5445445445	23.8053989043507;
42442.5935935936	24.0686228962846;
42492.6426426426	23.9105857019247;
42542.6916916917	23.9165506960867;
42592.7407407407	23.9754241418607;
42642.7897897898	23.8776167348849;
42692.8388388388	23.683661871467;
42742.8878878879	23.9879008857342;
42792.9369369369	23.8102202905886;
42842.985985986	23.7865514033256;
42893.035035035	23.7631475328284;
42943.0840840841	23.7701349542204;
42993.1331331331	23.5909818969491;
43043.1821821822	23.7261382422962;
43093.2312312312	23.945644233482;
43143.2802802803	23.6068543470679;
43193.3293293293	23.7215407955658;
43243.3783783784	23.9479993092011;
43293.4274274274	23.837873988461;
43343.4764764765	23.9701601481787;
43393.5255255255	23.9123571067039;
43443.5745745746	24.1332512421468;
43493.6236236236	23.8734344492866;
43543.6726726727	23.7030190174544;
43593.7217217217	23.9883303586633;
43643.7707707708	23.7185161413626;
43693.8198198198	23.8731347484703;
43743.8688688689	23.8588279935395;
43793.9179179179	23.6927292342179;
43843.966966967	23.7226687004574;
43894.016016016	23.9654053453566;
43944.0650650651	23.9824359039808;
43994.1141141141	23.9643086780799;
44044.1631631632	23.8550161024968;
44094.2122122122	23.8633100394839;
44144.2612612613	23.6339395568499;
44194.3103103103	23.8162668967873;
44244.3593593594	24.1019058712292;
44294.4084084084	23.7334800971791;
44344.4574574575	23.9921498185105;
44394.5065065065	23.6150173687488;
44444.5555555556	23.885279067041;
44494.6046046046	23.6567228851438;
44544.6536536537	23.6806526551565;
44594.7027027027	23.6500122486943;
44644.7517517518	23.896693986809;
44694.8008008008	23.8753060936729;
44744.8498498499	23.8031307121081;
44794.8988988989	23.9712453877048;
44844.9479479479	23.6647029444741;
44894.996996997	23.8371392445523;
44945.046046046	23.7115139272685;
44995.0950950951	24.1452964877976;
45045.1441441441	23.829613258164;
45095.1931931932	23.7403610888205;
45145.2422422422	23.8378383494769;
45195.2912912913	23.7399263184817;
45245.3403403403	23.9140548525469;
45295.3893893894	23.6533657812797;
45345.4384384384	23.7205522304626;
45395.4874874875	24.0061758334262;
45445.5365365365	23.767958285136;
45495.5855855856	23.8398321706744;
45545.6346346346	23.7872008651243;
45595.6836836837	23.9052662747977;
45645.7327327327	23.7970746775121;
45695.7817817818	23.7277002582802;
45745.8308308308	23.7451820836175;
45795.8798798799	23.6417044456577;
45845.9289289289	23.7229312146207;
45895.977977978	23.6755911580595;
45946.027027027	23.9197795093419;
45996.0760760761	23.8668974021889;
46046.1251251251	23.8707964249599;
46096.1741741742	23.930716629058;
46146.2232232232	24.01290315074;
46196.2722722723	23.844912552916;
46246.3213213213	23.7258160371663;
46296.3703703704	23.8601047042141;
46346.4194194194	23.7396865417519;
46396.4684684685	23.8587703470116;
46446.5175175175	23.7809178884554;
46496.5665665666	23.714538233529;
46546.6156156156	23.8774745920182;
46596.6646646647	23.7405313232943;
46646.7137137137	23.8965907915887;
46696.7627627628	23.7880220442571;
46746.8118118118	23.6236984132254;
46796.8608608609	23.481909897816;
46846.9099099099	23.9338600103789;
46896.958958959	23.7116685498987;
46947.008008008	23.9238181310547;
46997.0570570571	24.0759814056542;
47047.1061061061	23.8781743020607;
47097.1551551552	24.0259056564875;
47147.2042042042	24.1034106959394;
47197.2532532533	23.9476868176239;
47247.3023023023	24.1180440495081;
47297.3513513514	23.8268997125489;
47347.4004004004	24.0072747177222;
47397.4494494495	23.4700473529235;
47447.4984984985	23.8131190686024;
47497.5475475475	24.0361007755388;
47547.5965965966	23.7113608172373;
47597.6456456456	23.8113493508176;
47647.6946946947	23.7554361114767;
47697.7437437437	23.9535288834471;
47747.7927927928	23.9486718023856;
47797.8418418418	23.8074481932853;
47847.8908908909	23.829676275427;
47897.9399399399	23.8673789245656;
47947.988988989	23.85913591693;
47998.038038038	23.8073679808043;
48048.0870870871	24.0583544382667;
48098.1361361361	23.6516070980745;
48148.1851851852	23.6755134446847;
48198.2342342342	23.7343741365992;
48248.2832832833	24.3145091602829;
48298.3323323323	23.8610442110588;
48348.3813813814	23.8466513275387;
48398.4304304304	23.6351416047425;
48448.4794794795	23.9754251433052;
48498.5285285285	23.7718080098476;
48548.5775775776	24.0071161912338;
48598.6266266266	23.6624106049079;
48648.6756756757	23.7974079309969;
48698.7247247247	23.6734571324361;
48748.7737737738	23.6439042399052;
48798.8228228228	23.9277677410293;
48848.8718718719	23.7208466945754;
48898.9209209209	23.9598879323466;
48948.96996997	23.7687330325895;
48999.019019019	24.0509650693152;
49049.0680680681	24.0199703428496;
49099.1171171171	23.8284971458479;
49149.1661661662	23.8406747017828;
49199.2152152152	23.8047623661314;
49249.2642642643	23.8110667085872;
49299.3133133133	23.8408111278698;
49349.3623623624	23.9533822726256;
49399.4114114114	23.7347290020191;
49449.4604604605	23.9841399392605;
49499.5095095095	23.5946079458476;
49549.5585585586	23.7983193732096;
49599.6076076076	23.8826036305133;
49649.6566566567	24.0421603449106;
49699.7057057057	23.8532378118135;
49749.7547547548	23.8488859678775;
49799.8038038038	23.8854798403103;
49849.8528528529	23.7391003441584;
49899.9019019019	23.7872564934511;
49949.950950951	23.8663320582485;
50000	23.9872261432331];


B = [1	3.41807738302787;
51.049049049049	3.4914746204508;
101.098098098098	3.71521463984374;
151.147147147147	3.78973436451299;
201.196196196196	3.66744211549463;
251.245245245245	3.60046028900246;
301.294294294294	3.81114113686159;
351.343343343343	3.84353022202378;
401.392392392392	3.57128753508452;
451.441441441441	3.82368005034106;
501.490490490491	3.53785126658034;
551.53953953954	3.58901409970363;
601.588588588589	3.75827991409706;
651.637637637638	3.66132984030113;
701.686686686687	3.81845756898034;
751.735735735736	3.67994255652696;
801.784784784785	4.01281588323629;
851.833833833834	3.9876020786288;
901.882882882883	4.02097800291595;
951.931931931932	4.08379298146241;
1001.98098098098	3.9129815423879;
1052.03003003003	3.78313012076413;
1102.07907907908	4.14017698644006;
1152.12812812813	3.92047824474778;
1202.17717717718	3.83009341603835;
1252.22622622623	3.84262774050701;
1302.27527527528	3.86869698493539;
1352.32432432432	3.90225789585038;
1402.37337337337	3.81861026529391;
1452.42242242242	3.90823873848808;
1502.47147147147	3.96719247404543;
1552.52052052052	3.5870898294524;
1602.56956956957	3.99455344305238;
1652.61861861862	3.77035089438858;
1702.66766766767	4.08031405110386;
1752.71671671672	4.3503646653401;
1802.76576576577	4.15383077575847;
1852.81481481481	4.33828782140821;
1902.86386386386	4.32372915739257;
1952.91291291291	4.31580491644293;
2002.96196196196	4.36676309148197;
2053.01101101101	4.12704884955861;
2103.06006006006	4.10727613481489;
2153.10910910911	4.2664376071186;
2203.15815815816	4.14085550794476;
2253.20720720721	4.23357607625026;
2303.25625625626	4.31228102477948;
2353.30530530531	4.44189140204666;
2403.35435435435	4.44959030455574;
2453.4034034034	4.44456410678274;
2503.45245245245	4.12744489699351;
2553.5015015015	4.27546391387776;
2603.55055055055	4.44275420216614;
2653.5995995996	4.29635706768546;
2703.64864864865	4.13251366197585;
2753.6976976977	4.07698295636026;
2803.74674674675	4.26986641835476;
2853.7957957958	4.21607930777972;
2903.84484484484	4.40964133444124;
2953.89389389389	4.33536038522961;
3003.94294294294	4.30496348974885;
3053.99199199199	4.32948503778339;
3104.04104104104	4.40560977568469;
3154.09009009009	4.37248063223611;
3204.13913913914	4.30779625922539;
3254.18818818819	4.41162790138995;
3304.23723723724	4.27901368810166;
3354.28628628629	4.36513814816599;
3404.33533533534	4.28644712041316;
3454.38438438438	4.52846294467361;
3504.43343343343	4.39114575332444;
3554.48248248248	4.7078616376926;
3604.53153153153	4.34852608909425;
3654.58058058058	4.3783530637272;
3704.62962962963	4.62409830908545;
3754.67867867868	4.34265181560337;
3804.72772772773	4.73194600817753;
3854.77677677678	4.33032643245531;
3904.82582582583	4.39077847450846;
3954.87487487487	4.44371816689454;
4004.92392392392	4.6338019489083;
4054.97297297297	4.34678359688342;
4105.02202202202	4.45932603151991;
4155.07107107107	4.33190679600373;
4205.12012012012	4.38332171515461;
4255.16916916917	4.47596273529213;
4305.21821821822	4.69591106896485;
4355.26726726727	4.65304946249443;
4405.31631631632	4.66292649170044;
4455.36536536537	4.72342117451484;
4505.41441441441	4.64819330762222;
4555.46346346346	4.70211738760441;
4605.51251251251	4.62740096629048;
4655.56156156156	4.6710447952697;
4705.61061061061	4.74778952059005;
4755.65965965966	4.80931693198413;
4805.70870870871	4.63261921727828;
4855.75775775776	4.69407105741815;
4905.80680680681	4.59907188686903;
4955.85585585586	4.59855766346285;
5005.9049049049	4.56452941948074;
5055.95395395395	4.72954183096682;
5106.003003003	4.60081471820326;
5156.05205205205	4.90307402041388;
5206.1011011011	4.67563188813918;
5256.15015015015	4.76163474448014;
5306.1991991992	4.66161166340755;
5356.24824824825	4.84103601650414;
5406.2972972973	4.82503963570106;
5456.34634634635	4.59803652483781;
5506.3953953954	4.84295308042766;
5556.44444444444	4.71547932622652;
5606.49349349349	4.4808525076365;
5656.54254254254	4.73040731467498;
5706.59159159159	4.79691847436635;
5756.64064064064	4.83710773034332;
5806.68968968969	4.85049731102182;
5856.73873873874	4.82072614906192;
5906.78778778779	4.4341664939278;
5956.83683683684	4.77083359315656;
6006.88588588589	4.64332838981571;
6056.93493493493	4.63636061544893;
6106.98398398398	4.60875096631559;
6157.03303303303	4.52747817783387;
6207.08208208208	4.67506639396769;
6257.13113113113	5.03627147886131;
6307.18018018018	5.02622731303764;
6357.22922922923	4.91920884824473;
6407.27827827828	4.98609278469194;
6457.32732732733	4.97819856804274;
6507.37637637638	4.7459006629668;
6557.42542542543	4.89715657925888;
6607.47447447447	4.88597320066309;
6657.52352352352	5.09779587834706;
6707.57257257257	5.07431548505302;
6757.62162162162	4.97310909883132;
6807.67067067067	5.04778496114695;
6857.71971971972	4.93699748228855;
6907.76876876877	4.81022564064456;
6957.81781781782	4.85102680998557;
7007.86686686687	5.0164146424648;
7057.91591591592	4.9373534740175;
7107.96496496496	4.78874720765743;
7158.01401401401	5.01560047186126;
7208.06306306306	4.85178600663509;
7258.11211211211	5.09629284833736;
7308.16116116116	5.01590888532347;
7358.21021021021	4.99337163259158;
7408.25925925926	5.02138076925302;
7458.30830830831	4.90812877234821;
7508.35735735736	4.97342380927044;
7558.40640640641	4.86583220042653;
7608.45545545546	4.93227866308744;
7658.5045045045	5.1987213893538;
7708.55355355355	5.00065886560398;
7758.6026026026	4.90473444181503;
7808.65165165165	4.99493631687498;
7858.7007007007	5.03738212097839;
7908.74974974975	5.26495138672103;
7958.7987987988	4.95280754920043;
8008.84784784785	4.8443039308988;
8058.8968968969	4.85495271320826;
8108.94594594595	4.92014297167143;
8158.994994995	4.94285410325799;
8209.04404404404	4.98036898889993;
8259.09309309309	5.11300059697055;
8309.14214214214	5.16109610634243;
8359.19119119119	4.9990286376599;
8409.24024024024	4.73113675670776;
8459.28928928929	4.93919025675393;
8509.33833833834	4.91106608110522;
8559.38738738739	5.04051380357337;
8609.43643643644	5.12343069171365;
8659.48548548549	4.96364705797116;
8709.53453453453	4.96170293801479;
8759.58358358358	4.97704070841545;
8809.63263263263	5.09267220311472;
8859.68168168168	5.14820469520027;
8909.73073073073	4.86966387176198;
8959.77977977978	5.11913584336937;
9009.82882882883	5.22018846035705;
9059.87787787788	5.07083922572979;
9109.92692692693	4.84921031508526;
9159.97597597598	5.05745853604081;
9210.02502502502	4.89621583746468;
9260.07407407407	5.09084879383598;
9310.12312312312	5.03891600157367;
9360.17217217217	5.04221907189464;
9410.22122122122	5.07380380670884;
9460.27027027027	4.96955543481186;
9510.31931931932	5.11963250287822;
9560.36836836837	5.0497005340794;
9610.41741741742	5.16289402444774;
9660.46646646647	4.97278159222071;
9710.51551551552	5.21898192796301;
9760.56456456457	5.1136725070883;
9810.61361361361	5.13468612410517;
9860.66266266266	5.17803031685306;
9910.71171171171	5.16456541486289;
9960.76076076076	5.18735391312429;
10010.8098098098	4.93229295642315;
10060.8588588589	5.11488621755928;
10110.9079079079	5.32506635360555;
10160.956956957	5.03402279281877;
10211.006006006	5.0656031167072;
10261.0550550551	4.99527315243505;
10311.1041041041	4.87003804439841;
10361.1531531532	5.00998722129743;
10411.2022022022	5.13788281857622;
10461.2512512513	5.14615382199956;
10511.3003003003	5.26386606904544;
10561.3493493493	5.03479040911746;
10611.3983983984	5.3617320781339;
10661.4474474474	5.33387453899906;
10711.4964964965	5.21415850221385;
10761.5455455455	5.18029562381691;
10811.5945945946	5.080873869183;
10861.6436436436	4.97774015517083;
10911.6926926927	5.37203854460401;
10961.7417417417	5.14102436676017;
11011.7907907908	5.05568735499202;
11061.8398398398	5.07776350150144;
11111.8888888889	5.22219219393912;
11161.9379379379	4.98131047696944;
11211.986986987	5.32896486388279;
11262.036036036	5.14107598505685;
11312.0850850851	5.11176081761714;
11362.1341341341	5.40146264587923;
11412.1831831832	5.31845000718143;
11462.2322322322	5.26050036766373;
11512.2812812813	5.38176768012136;
11562.3303303303	5.17187282545343;
11612.3793793794	5.19835979470876;
11662.4284284284	5.22172551603374;
11712.4774774775	5.25513996814437;
11762.5265265265	5.3017853668315;
11812.5755755756	5.35582129275643;
11862.6246246246	5.21028108175345;
11912.6736736737	5.22961764057725;
11962.7227227227	5.44706111598489;
12012.7717717718	5.25311984466687;
12062.8208208208	5.40913253046671;
12112.8698698699	5.14067112956806;
12162.9189189189	5.26536370046293;
12212.967967968	5.31192940628671;
12263.017017017	5.23249846174628;
12313.0660660661	5.41055993715821;
12363.1151151151	5.29310337210469;
12413.1641641642	5.16193175969753;
12463.2132132132	5.34793354393612;
12513.2622622623	5.5102641117199;
12563.3113113113	5.08179987875438;
12613.3603603604	5.52586461696175;
12663.4094094094	5.29546624841509;
12713.4584584585	5.33550847378829;
12763.5075075075	5.17831267111163;
12813.5565565566	5.56899951571124;
12863.6056056056	5.02324082269694;
12913.6546546547	5.26290050209783;
12963.7037037037	5.37597527292956;
13013.7527527528	5.25494570376042;
13063.8018018018	5.07913024875597;
13113.8508508509	5.16798668380521;
13163.8998998999	5.43321257309583;
13213.9489489489	5.1880072235026;
13263.997997998	5.58124346461353;
13314.047047047	5.47741158258351;
13364.0960960961	5.17671762948293;
13414.1451451451	5.03788844218826;
13464.1941941942	5.24115866108837;
13514.2432432432	5.2258097818846;
13564.2922922923	5.18084057938737;
13614.3413413413	5.2022318022982;
13664.3903903904	5.29554133658543;
13714.4394394394	5.37672675229101;
13764.4884884885	5.26710056452311;
13814.5375375375	5.23972525638946;
13864.5865865866	5.22887655160984;
13914.6356356356	5.39771745244681;
13964.6846846847	5.30766446172578;
14014.7337337337	5.11045694025533;
14064.7827827828	5.32520105674703;
14114.8318318318	5.43409805496145;
14164.8808808809	5.40680055800188;
14214.9299299299	5.38492635209671;
14264.978978979	5.38895436310298;
14315.028028028	5.12253057969802;
14365.0770770771	5.37868577521184;
14415.1261261261	5.22573861461349;
14465.1751751752	5.41282552895552;
14515.2242242242	5.2704266706764;
14565.2732732733	5.22163051429334;
14615.3223223223	5.28730414254267;
14665.3713713714	5.23946660981873;
14715.4204204204	5.24013251704129;
14765.4694694695	5.42686568117562;
14815.5185185185	5.17464632277214;
14865.5675675676	5.29760615585414;
14915.6166166166	5.32360122522384;
14965.6656656657	5.21764635892951;
15015.7147147147	5.40985638849742;
15065.7637637638	5.22558601327418;
15115.8128128128	5.08687225953622;
15165.8618618619	5.25252873890623;
15215.9109109109	4.93358266382477;
15265.95995996	5.28131592807769;
15316.009009009	5.19745703874706;
15366.0580580581	5.27103487506079;
15416.1071071071	5.33420048105715;
15466.1561561562	5.25664953390352;
15516.2052052052	5.49058068046831;
15566.2542542543	5.13605771011114;
15616.3033033033	5.26862827753746;
15666.3523523524	5.33070528181029;
15716.4014014014	5.28354673798434;
15766.4504504505	5.30993459741397;
15816.4994994995	5.09384544989847;
15866.5485485485	5.18403632272512;
15916.5975975976	5.54845111184181;
15966.6466466466	5.26952105480336;
16016.6956956957	5.18260831803827;
16066.7447447447	5.36677790112299;
16116.7937937938	5.10185325660166;
16166.8428428428	5.29166162807459;
16216.8918918919	5.07253329293909;
16266.9409409409	5.44656393244939;
16316.98998999	5.16262651025084;
16367.039039039	5.25511277129724;
16417.0880880881	5.20003936035158;
16467.1371371371	5.19893684303176;
16517.1861861862	5.32461817305816;
16567.2352352352	5.194870034321;
16617.2842842843	5.41320047181439;
16667.3333333333	5.2261464752969;
16717.3823823824	5.40986498734038;
16767.4314314314	5.17762676160729;
16817.4804804805	5.33576032319891;
16867.5295295295	5.46542447668912;
16917.5785785786	5.18539723332228;
16967.6276276276	5.45440473619067;
17017.6766766767	5.34437700595798;
17067.7257257257	5.39887003226996;
17117.7747747748	5.19709711369891;
17167.8238238238	5.46498576450151;
17217.8728728729	5.35727111753451;
17267.9219219219	5.14096513356982;
17317.970970971	5.26928541451814;
17368.02002002	5.35925010086025;
17418.0690690691	5.38288628457519;
17468.1181181181	5.29588037499712;
17518.1671671672	5.57107814003713;
17568.2162162162	5.31946017395889;
17618.2652652653	5.51464947648961;
17668.3143143143	5.39056399539429;
17718.3633633634	5.25820151536302;
17768.4124124124	5.76538957497538;
17818.4614614615	5.31647765942106;
17868.5105105105	5.46083205965947;
17918.5595595596	5.42016125404482;
17968.6086086086	5.26701810090427;
18018.6576576577	5.24660210082061;
18068.7067067067	5.68220558780296;
18118.7557557558	5.52717201972139;
18168.8048048048	5.39442456144172;
18218.8538538539	5.28393007395098;
18268.9029029029	5.36958807539768;
18318.951951952	5.33999544199955;
18369.001001001	5.14184009462183;
18419.05005005	5.55065775775766;
18469.0990990991	5.30652993029271;
18519.1481481481	5.27776420754159;
18569.1971971972	5.16799584742364;
18619.2462462462	5.44819647047511;
18669.2952952953	5.35041067466504;
18719.3443443443	5.4637490686344;
18769.3933933934	5.24409615070523;
18819.4424424424	5.31326020385509;
18869.4914914915	5.68416056104523;
18919.5405405405	5.46573239751987;
18969.5895895896	5.35820325188946;
19019.6386386386	5.39594900487711;
19069.6876876877	5.43190285174711;
19119.7367367367	5.43941334229263;
19169.7857857858	5.49642693885592;
19219.8348348348	5.51283351909993;
19269.8838838839	5.47618419541297;
19319.9329329329	5.37206852215987;
19369.981981982	5.0922130857254;
19420.031031031	5.48603235891736;
19470.0800800801	5.29249513535165;
19520.1291291291	5.39135687990668;
19570.1781781782	5.42690791347151;
19620.2272272272	5.4084941797403;
19670.2762762763	5.37214151483624;
19720.3253253253	5.16851189993407;
19770.3743743744	5.49249700991859;
19820.4234234234	5.52785515171402;
19870.4724724725	5.48348820411173;
19920.5215215215	5.51532075460719;
19970.5705705706	5.53794812528115;
20020.6196196196	5.38678947131142;
20070.6686686687	5.459927780274;
20120.7177177177	5.38468189123928;
20170.7667667668	5.59002311363442;
20220.8158158158	5.57121738522921;
20270.8648648649	5.38147953763431;
20320.9139139139	5.59223821858262;
20370.962962963	5.40464902493282;
20421.012012012	5.35259672786764;
20471.0610610611	5.41054510689959;
20521.1101101101	5.29466338154639;
20571.1591591592	5.40101530128444;
20621.2082082082	5.58836092383233;
20671.2572572573	5.42755774339779;
20721.3063063063	5.40509185136583;
20771.3553553554	5.35665301341432;
20821.4044044044	5.5060347371134;
20871.4534534535	5.36543581447392;
20921.5025025025	5.47165038574022;
20971.5515515516	5.36652852388733;
21021.6006006006	5.28971426120312;
21071.6496496497	5.4188637111814;
21121.6986986987	5.25386599065728;
21171.7477477477	5.68155322765205;
21221.7967967968	5.37487226184311;
21271.8458458458	5.25137625930285;
21321.8948948949	5.54691402014496;
21371.9439439439	5.48444492910144;
21421.992992993	5.51927287543781;
21472.042042042	5.32036466619824;
21522.0910910911	5.21541822101778;
21572.1401401401	5.55510632752944;
21622.1891891892	5.53631823756232;
21672.2382382382	5.39304374651854;
21722.2872872873	5.55271179301434;
21772.3363363363	5.47860238809954;
21822.3853853854	5.37235605727356;
21872.4344344344	5.3866386700399;
21922.4834834835	5.51255861213877;
21972.5325325325	5.41365311999158;
22022.5815815816	5.37194873409436;
22072.6306306306	5.41307242191332;
22122.6796796797	5.57708242319843;
22172.7287287287	5.54521524400497;
22222.7777777778	5.53883744326338;
22272.8268268268	5.32240903778887;
22322.8758758759	5.42404163404165;
22372.9249249249	5.51296449060768;
22422.973973974	5.28000201548918;
22473.023023023	5.80438422324324;
22523.0720720721	5.43014408869332;
22573.1211211211	5.44123213571502;
22623.1701701702	5.57924053193435;
22673.2192192192	5.63250438427817;
22723.2682682683	5.36802473628841;
22773.3173173173	5.31338777767275;
22823.3663663664	5.48122879169324;
22873.4154154154	5.24129304358922;
22923.4644644645	5.32344066677035;
22973.5135135135	5.29201373219109;
23023.5625625626	5.36828928967664;
23073.6116116116	5.46577859108505;
23123.6606606607	5.57901146865962;
23173.7097097097	5.22317161925094;
23223.7587587588	5.66152620612723;
23273.8078078078	5.44662141619038;
23323.8568568569	5.60637027138883;
23373.9059059059	5.33926973138419;
23423.954954955	5.59332990495407;
23474.004004004	5.649739607395;
23524.0530530531	5.42619894712239;
23574.1021021021	5.6032051879313;
23624.1511511512	5.66301942864667;
23674.2002002002	5.5105916441234;
23724.2492492492	5.56357656228158;
23774.2982982983	5.64134178154241;
23824.3473473473	5.49969851558885;
23874.3963963964	5.22058975120355;
23924.4454454454	5.57454429760831;
23974.4944944945	5.3883497817975;
24024.5435435435	5.60963677694299;
24074.5925925926	5.41632590660601;
24124.6416416416	5.6578048579035;
24174.6906906907	5.45362621421844;
24224.7397397397	5.57170528300317;
24274.7887887888	5.54390203968315;
24324.8378378378	5.47299623294102;
24374.8868868869	5.59140585856661;
24424.9359359359	5.25482000398133;
24474.984984985	5.49175529775155;
24525.034034034	5.4653848898762;
24575.0830830831	5.56937982132548;
24625.1321321321	5.33874012828074;
24675.1811811812	5.36521146244484;
24725.2302302302	5.44780238307851;
24775.2792792793	5.68442838234192;
24825.3283283283	5.44536938628249;
24875.3773773774	5.49073717349715;
24925.4264264264	5.39380187272147;
24975.4754754755	5.24300489346663;
25025.5245245245	5.50638096783986;
25075.5735735736	5.71077213612252;
25125.6226226226	5.46702969189559;
25175.6716716717	5.24561931156074;
25225.7207207207	5.38826825293244;
25275.7697697698	5.38422409947411;
25325.8188188188	5.40407908456663;
25375.8678678679	5.49005084192081;
25425.9169169169	5.54021058213545;
25475.965965966	5.52924085717337;
25526.015015015	5.39913222699276;
25576.0640640641	5.32467296625842;
25626.1131131131	5.51611519475953;
25676.1621621622	5.46846227383668;
25726.2112112112	5.56532599653165;
25776.2602602603	5.4681668483277;
25826.3093093093	5.63794384714173;
25876.3583583584	5.50110796932183;
25926.4074074074	5.27989652094399;
25976.4564564565	5.50176601466636;
26026.5055055055	5.42964348215959;
26076.5545545546	5.27626960318515;
26126.6036036036	5.55807791927384;
26176.6526526527	5.33307676695207;
26226.7017017017	5.42930197919718;
26276.7507507508	5.48649908245628;
26326.7997997998	5.3282762426747;
26376.8488488488	5.47824652870311;
26426.8978978979	5.65588955694059;
26476.9469469469	5.54890834982816;
26526.995995996	5.37185365235309;
26577.045045045	5.48265435114041;
26627.0940940941	5.38685534881713;
26677.1431431431	5.65588558457856;
26727.1921921922	5.63851945803379;
26777.2412412412	5.4329202371275;
26827.2902902903	5.27961925755993;
26877.3393393393	5.25085698681592;
26927.3883883884	5.62538169391735;
26977.4374374374	5.67330078959523;
27027.4864864865	5.58486125613069;
27077.5355355355	5.36709160921569;
27127.5845845846	5.57666282620388;
27177.6336336336	5.56193016973851;
27227.6826826827	5.30064772607812;
27277.7317317317	5.40427157432172;
27327.7807807808	5.62714861355184;
27377.8298298298	5.28103873379389;
27427.8788788789	5.31664066286848;
27477.9279279279	5.55599776823634;
27527.976976977	5.2514053003523;
27578.026026026	5.68183496571678;
27628.0750750751	5.4651444881191;
27678.1241241241	5.68967332674146;
27728.1731731732	5.49226719665319;
27778.2222222222	5.49790563798331;
27828.2712712713	5.30817229178504;
27878.3203203203	5.59786900206434;
27928.3693693694	5.52391668898438;
27978.4184184184	5.56254446484218;
28028.4674674675	5.47162508623756;
28078.5165165165	5.58037462891395;
28128.5655655656	5.24119451938528;
28178.6146146146	5.53065155127655;
28228.6636636637	5.23353150557115;
28278.7127127127	5.36210719728461;
28328.7617617618	5.28141460048665;
28378.8108108108	5.57427397867811;
28428.8598598599	5.32116390196441;
28478.9089089089	5.52583411624262;
28528.957957958	5.6881722230489;
28579.007007007	5.47195922661484;
28629.0560560561	5.53980387241331;
28679.1051051051	5.48241613278807;
28729.1541541542	5.40072958999778;
28779.2032032032	5.40598256967312;
28829.2522522523	5.64296693976556;
28879.3013013013	5.53794473116711;
28929.3503503503	5.55940108200602;
28979.3993993994	5.40189935202196;
29029.4484484484	5.54014572997089;
29079.4974974975	5.60608184228932;
29129.5465465465	5.39704361921805;
29179.5955955956	5.77635826320492;
29229.6446446446	5.45073501130827;
29279.6936936937	5.52981556544527;
29329.7427427427	5.41757489534549;
29379.7917917918	5.39037982247776;
29429.8408408408	5.40044604562792;
29479.8898898899	5.42017698991173;
29529.9389389389	5.55156971846148;
29579.987987988	5.40438160132567;
29630.037037037	5.26193707734839;
29680.0860860861	5.34173036455823;
29730.1351351351	5.19958831334659;
29780.1841841842	5.43185254354379;
29830.2332332332	5.67563223199908;
29880.2822822823	5.48694617828667;
29930.3313313313	5.55724245765658;
29980.3803803804	5.43434065381195;
30030.4294294294	5.50006178223845;
30080.4784784785	5.69555108325159;
30130.5275275275	5.56397662584855;
30180.5765765766	5.53113784565881;
30230.6256256256	5.26290862456338;
30280.6746746747	5.40257672406719;
30330.7237237237	5.58885641137937;
30380.7727727728	5.4396797050187;
30430.8218218218	5.4522825631853;
30480.8708708709	5.42308704134801;
30530.9199199199	5.49044616922775;
30580.968968969	5.45366774988575;
30631.018018018	5.31038596396085;
30681.0670670671	5.54428482424478;
30731.1161161161	5.63383215906592;
30781.1651651652	5.40709760993564;
30831.2142142142	5.65508363237824;
30881.2632632633	5.60321333408033;
30931.3123123123	5.4926787909971;
30981.3613613614	5.51573037937952;
31031.4104104104	5.44529353679937;
31081.4594594595	5.48519867763095;
31131.5085085085	5.37977562503942;
31181.5575575576	5.5368525355028;
31231.6066066066	5.36785111645106;
31281.6556556557	5.56743167481425;
31331.7047047047	5.49159396909339;
31381.7537537538	5.2507005872094;
31431.8028028028	5.58903036986154;
31481.8518518519	5.51783476888764;
31531.9009009009	5.39954091361585;
31581.94994995	5.29377660868806;
31631.998998999	5.51016256188484;
31682.048048048	5.34598957345195;
31732.0970970971	5.31751084274656;
31782.1461461461	5.23936661296701;
31832.1951951952	5.37832621459398;
31882.2442442442	5.437100857283;
31932.2932932933	5.49654080695515;
31982.3423423423	5.46056401827558;
32032.3913913914	5.44234776344486;
32082.4404404404	5.47328268586496;
32132.4894894895	5.37012103275664;
32182.5385385385	5.34797877379663;
32232.5875875876	5.44767356642697;
32282.6366366366	5.52947738268027;
32332.6856856857	5.47316252460902;
32382.7347347347	5.46444444247575;
32432.7837837838	5.52838182126488;
32482.8328328328	5.43372691323979;
32532.8818818819	5.39795559666162;
32582.9309309309	5.55533517965365;
32632.97997998	5.57543426428727;
32683.029029029	5.67811806547655;
32733.0780780781	5.43377856055962;
32783.1271271271	5.42115078433181;
32833.1761761762	5.45856709511935;
32883.2252252252	5.60513468294276;
32933.2742742743	5.17883801976096;
32983.3233233233	5.60809629547284;
33033.3723723724	5.50668152870325;
33083.4214214214	5.50216526100423;
33133.4704704705	5.42427838944359;
33183.5195195195	5.64484519689707;
33233.5685685686	5.65281113904569;
33283.6176176176	5.48617915293879;
33333.6666666667	5.63881068024142;
33383.7157157157	5.531912323332;
33433.7647647648	5.4151400339227;
33483.8138138138	5.61204254662786;
33533.8628628629	5.38024013773551;
33583.9119119119	5.56500663555435;
33633.960960961	5.60037916442273;
33684.01001001	5.45287496332248;
33734.0590590591	5.37050828851688;
33784.1081081081	5.69696556218829;
33834.1571571572	5.52851911289177;
33884.2062062062	5.29420584408386;
33934.2552552553	5.52543439680023;
33984.3043043043	5.69545153738151;
34034.3533533534	5.47536043450062;
34084.4024024024	5.55925741275776;
34134.4514514515	5.24441973897848;
34184.5005005005	5.4271603817784;
34234.5495495495	5.35243770392792;
34284.5985985986	5.51273457179056;
34334.6476476476	5.51946858646655;
34384.6966966967	5.6771290578513;
34434.7457457457	5.25533823705029;
34484.7947947948	5.26821754761455;
34534.8438438438	5.47673755748863;
34584.8928928929	5.59332932711168;
34634.9419419419	5.25275735157528;
34684.990990991	5.49686479179412;
34735.04004004	5.33642870778378;
34785.0890890891	5.84315279853823;
34835.1381381381	5.42500689709042;
34885.1871871872	5.44773688219335;
34935.2362362362	5.56157685721976;
34985.2852852853	5.41915978242465;
35035.3343343343	5.30265040894238;
35085.3833833834	5.37060606645632;
35135.4324324324	5.32948940023855;
35185.4814814815	5.70622460863372;
35235.5305305305	5.51989219708852;
35285.5795795796	5.53218958609695;
35335.6286286286	5.4892706534976;
35385.6776776777	5.53653756857172;
35435.7267267267	5.63575893979373;
35485.7757757758	5.62781674748192;
35535.8248248248	5.43537698189538;
35585.8738738739	5.44798504827869;
35635.9229229229	5.52437629152715;
35685.971971972	5.55501072647009;
35736.021021021	5.47982562223336;
35786.0700700701	5.78208490952821;
35836.1191191191	5.64247407861658;
35886.1681681682	5.47740237356701;
35936.2172172172	5.49738276932601;
35986.2662662663	5.53293561894681;
36036.3153153153	5.51287577047189;
36086.3643643644	5.70620430959501;
36136.4134134134	5.37770987878425;
36186.4624624625	5.6147218225558;
36236.5115115115	5.60942108770572;
36286.5605605606	5.32540321831229;
36336.6096096096	5.35263823805173;
36386.6586586587	5.76082914680693;
36436.7077077077	5.75074701509216;
36486.7567567568	5.57167242590554;
36536.8058058058	5.60432992211307;
36586.8548548549	5.54008822055302;
36636.9039039039	5.56701382420635;
36686.952952953	5.41054755686334;
36737.002002002	5.5477233402227;
36787.0510510511	5.58105720808984;
36837.1001001001	5.48488973227907;
36887.1491491491	5.47285957264273;
36937.1981981982	5.33758328693281;
36987.2472472472	5.4491822076619;
37037.2962962963	5.61482873296225;
37087.3453453453	5.48489052261181;
37137.3943943944	5.51704524710826;
37187.4434434434	5.4535024471665;
37237.4924924925	5.53491482593882;
37287.5415415415	5.38022605364499;
37337.5905905906	5.5693195469334;
37387.6396396396	5.6456149210279;
37437.6886886887	5.50514700604353;
37487.7377377377	5.33694938614425;
37537.7867867868	5.5446799602171;
37587.8358358358	5.30779962440959;
37637.8848848849	5.66548401287341;
37687.9339339339	5.49111792575074;
37737.982982983	5.34455548863117;
37788.032032032	5.44477268897058;
37838.0810810811	5.52209906801238;
37888.1301301301	5.39732313415407;
37938.1791791792	5.50034064117236;
37988.2282282282	5.30648597949367;
38038.2772772773	5.30497104549644;
38088.3263263263	5.52052014289279;
38138.3753753754	5.46692803285221;
38188.4244244244	5.4984109019955;
38238.4734734735	5.63331821350233;
38288.5225225225	5.52080432044866;
38338.5715715716	5.35756785830385;
38388.6206206206	5.58776002451496;
38438.6696696697	5.73888618005454;
38488.7187187187	5.44820419002596;
38538.7677677678	5.15258795504528;
38588.8168168168	5.39028124108233;
38638.8658658659	5.41583875021552;
38688.9149149149	5.43397638792047;
38738.963963964	5.29886884909821;
38789.013013013	5.46372844523679;
38839.0620620621	5.46914022098241;
38889.1111111111	5.16850336353169;
38939.1601601602	5.28157551737541;
38989.2092092092	5.40087671780964;
39039.2582582583	5.43831795016744;
39089.3073073073	5.62045487439763;
39139.3563563564	5.42380453618055;
39189.4054054054	5.46882022231698;
39239.4544544545	5.58885166514746;
39289.5035035035	5.35429597218556;
39339.5525525526	5.61425890441027;
39389.6016016016	5.38796064938537;
39439.6506506506	5.37718881773257;
39489.6996996997	5.49779672915207;
39539.7487487487	5.3056465214632;
39589.7977977978	5.40952851788001;
39639.8468468468	5.4566951941788;
39689.8958958959	5.20581223221528;
39739.9449449449	5.66458107973195;
39789.993993994	5.39698691889381;
39840.043043043	5.48546193848665;
39890.0920920921	5.57239355111726;
39940.1411411411	5.42975941452144;
39990.1901901902	5.50648170264169;
40040.2392392392	5.47708803453193;
40090.2882882883	5.29190127399544;
40140.3373373373	5.43996859345721;
40190.3863863864	5.45485974189201;
40240.4354354354	5.39896481427722;
40290.4844844845	5.55796707150147;
40340.5335335335	5.56962177494874;
40390.5825825826	5.699009359297;
40440.6316316316	5.53275975469439;
40490.6806806807	5.39819147484329;
40540.7297297297	5.55216002500235;
40590.7787787788	5.61372854636158;
40640.8278278278	5.46296915530554;
40690.8768768769	5.3679247558909;
40740.9259259259	5.56636146064017;
40790.974974975	5.64144283583643;
40841.024024024	5.5058599592443;
40891.0730730731	5.47425354388526;
40941.1221221221	5.44956118897218;
40991.1711711712	5.47698068234943;
41041.2202202202	5.45765259427307;
41091.2692692693	5.83248318116605;
41141.3183183183	5.48932451791095;
41191.3673673674	5.19678770289961;
41241.4164164164	5.55584854772484;
41291.4654654655	5.31355977241894;
41341.5145145145	5.38793861685075;
41391.5635635636	5.47316221694128;
41441.6126126126	5.50043517304296;
41491.6616616617	5.61798536176188;
41541.7107107107	5.41099947040545;
41591.7597597598	5.5570220895035;
41641.8088088088	5.3573511172953;
41691.8578578579	5.56676260848206;
41741.9069069069	5.38018010898944;
41791.955955956	5.41892944468798;
41842.005005005	5.60102373536478;
41892.0540540541	5.5535219373319;
41942.1031031031	5.36148551100467;
41992.1521521521	5.57065233394393;
42042.2012012012	5.28742006581398;
42092.2502502503	5.60703061834788;
42142.2992992993	5.52583223696401;
42192.3483483484	5.60002485695662;
42242.3973973974	5.4471687596284;
42292.4464464464	5.45429183124348;
42342.4954954955	5.54901711386367;
42392.5445445445	5.60797208569004;
42442.5935935936	5.54889916536565;
42492.6426426426	5.68051302268196;
42542.6916916917	5.52421628104563;
42592.7407407407	5.46211700775576;
42642.7897897898	5.57680334379029;
42692.8388388388	5.57623186116601;
42742.8878878879	5.49713083007371;
42792.9369369369	5.54806647857394;
42842.985985986	5.65964152773432;
42893.035035035	5.58364338684051;
42943.0840840841	5.84654072882402;
42993.1331331331	5.60280554201072;
43043.1821821822	5.49474397834286;
43093.2312312312	5.43915184485556;
43143.2802802803	5.42441641475005;
43193.3293293293	5.42451153469756;
43243.3783783784	5.63006938345061;
43293.4274274274	5.39049391227776;
43343.4764764765	5.35330685604096;
43393.5255255255	5.30427830173999;
43443.5745745746	5.40762629446451;
43493.6236236236	5.57416214818857;
43543.6726726727	5.70835955951121;
43593.7217217217	5.49095568860862;
43643.7707707708	5.7728220837502;
43693.8198198198	5.43846966890543;
43743.8688688689	5.50596496255514;
43793.9179179179	5.61370593956258;
43843.966966967	5.39795995087034;
43894.016016016	5.7644413224574;
43944.0650650651	5.48547898915746;
43994.1141141141	5.39607672113737;
44044.1631631632	5.45138334405007;
44094.2122122122	5.61841412380925;
44144.2612612613	5.25432535077724;
44194.3103103103	5.50271607901316;
44244.3593593594	5.5530597417023;
44294.4084084084	5.37346007473385;
44344.4574574575	5.28059319998849;
44394.5065065065	5.3703764843552;
44444.5555555556	5.56434031250257;
44494.6046046046	5.50247044196023;
44544.6536536537	5.59535227652828;
44594.7027027027	5.55903918572552;
44644.7517517518	5.39622666670605;
44694.8008008008	5.26154373041428;
44744.8498498499	5.39964112498359;
44794.8988988989	5.55140631354003;
44844.9479479479	5.39868379430808;
44894.996996997	5.59178117487596;
44945.046046046	5.59364922713898;
44995.0950950951	5.43114880583365;
45045.1441441441	5.65421602175434;
45095.1931931932	5.47088754740059;
45145.2422422422	5.55610975156867;
45195.2912912913	5.36889606691169;
45245.3403403403	5.40065284390472;
45295.3893893894	5.48403807330863;
45345.4384384384	5.60894634912639;
45395.4874874875	5.38595531473509;
45445.5365365365	5.63309700619639;
45495.5855855856	5.68838238641464;
45545.6346346346	5.50132010825329;
45595.6836836837	5.37141012513319;
45645.7327327327	5.50606907903848;
45695.7817817818	5.62085629844726;
45745.8308308308	5.44452212769107;
45795.8798798799	5.56258202883746;
45845.9289289289	5.49771653007219;
45895.977977978	5.33145961260239;
45946.027027027	5.60624006055455;
45996.0760760761	5.63868808445837;
46046.1251251251	5.68779695898834;
46096.1741741742	5.5584061310448;
46146.2232232232	5.49455943437727;
46196.2722722723	5.42406185710845;
46246.3213213213	5.47460926710157;
46296.3703703704	5.42241624093776;
46346.4194194194	5.17339918209897;
46396.4684684685	5.57523481134016;
46446.5175175175	5.47785275733178;
46496.5665665666	5.45104837079767;
46546.6156156156	5.56465514069572;
46596.6646646647	5.43272362191169;
46646.7137137137	5.77479460767453;
46696.7627627628	5.45934133850507;
46746.8118118118	5.43584792288704;
46796.8608608609	5.40074512674427;
46846.9099099099	5.80025464708501;
46896.958958959	5.46707540035575;
46947.008008008	5.51262593451209;
46997.0570570571	5.6062084333987;
47047.1061061061	5.65644841081439;
47097.1551551552	5.22895023340819;
47147.2042042042	5.72849471590953;
47197.2532532533	5.51936503631522;
47247.3023023023	5.37024955943919;
47297.3513513514	5.38520905706393;
47347.4004004004	5.58221472157434;
47397.4494494495	5.53012058117595;
47447.4984984985	5.51295757383197;
47497.5475475475	5.552907956817;
47547.5965965966	5.70933315771223;
47597.6456456456	5.45139323559302;
47647.6946946947	5.60632685572618;
47697.7437437437	5.46970567395652;
47747.7927927928	5.51377101471252;
47797.8418418418	5.38501900612775;
47847.8908908909	5.68736738912668;
47897.9399399399	5.54552877606672;
47947.988988989	5.39024558852861;
47998.038038038	5.48411683352384;
48048.0870870871	5.5395246940031;
48098.1361361361	5.60890735311653;
48148.1851851852	5.31531132225866;
48198.2342342342	5.67777957283074;
48248.2832832833	5.472076603416;
48298.3323323323	5.43088399745705;
48348.3813813814	5.36563144742194;
48398.4304304304	5.62607231395178;
48448.4794794795	5.36138459104729;
48498.5285285285	5.40144671087797;
48548.5775775776	5.57028621696748;
48598.6266266266	5.42744666614845;
48648.6756756757	5.47136498389989;
48698.7247247247	5.552916853157;
48748.7737737738	5.47603343414529;
48798.8228228228	5.5618226038502;
48848.8718718719	5.38092250246485;
48898.9209209209	5.42693800550469;
48948.96996997	5.38983207911418;
48999.019019019	5.50799718543902;
49049.0680680681	5.51292080111329;
49099.1171171171	5.57698495292081;
49149.1661661662	5.51039295557204;
49199.2152152152	5.67016694623856;
49249.2642642643	5.5610252446076;
49299.3133133133	5.45415609956149;
49349.3623623624	5.51471042377546;
49399.4114114114	5.63339121386649;
49449.4604604605	5.70669089267265;
49499.5095095095	5.53245090862925;
49549.5585585586	5.56601727584473;
49599.6076076076	5.5554698577161;
49649.6566566567	5.49567495255596;
49699.7057057057	5.45367744739227;
49749.7547547548	5.69041662868456;
49799.8038038038	5.41390315992854;
49849.8528528529	5.53031023019989;
49899.9019019019	5.52100199089806;
49949.950950951	5.45861778787484;
50000	5.25891281833779];
